Disentangled Sequential Autoencoder

We present a VAE architecture for encoding and generating high dimensional sequential data, such as video or audio. Our deep generative model learns a latent representation of the data which is split into a static and dynamic part, allowing us to approximately disentangle latent time-dependent features (dynamics) from features which are preserved over time (content). This architecture gives us partial control over generating content and dynamics by conditioning on either one of these sets of features. In our experiments on artificially generated cartoon video clips and voice recordings, we show that we can convert the content of a given sequence into another one by such content swapping. For audio, this allows us to convert a male speaker into a female speaker and vice versa, while for video we can separately manipulate shapes and dynamics. Furthermore, we give empirical evidence for the hypothesis that stochastic RNNs as latent state models are more efficient at compressing and generating long sequences than deterministic ones, which may be relevant for applications in video compression.

==> quickdraw_test.tex <==
\subsection{Human drawing data: QuickDraw shapes}
The third experiment investigates a sequential dataset that has very different characteristics: human drawing. In this case an object is drew on a paper, and the strokes of that drawing is tracked as a time-series. Here, the identity of the object is defined by the whole sequences, which is distinct from the video/speech data tests that the object identity is entailed as time-invariant information. Still, we conjecture that there exists time-invariant information in the drawing sequence, e.g.~the drawing style of an user, and examine our model on a hand drawing dataset as the following.

\paragraph{Dataset and pre-processing.}
QuickDraw \citep{quick2016} is a dataset of vector drawings obtained from an online drawing game \emph{Quick, Draw!} where the player needs to draw a particular object in less than 20 seconds. For the purpose of our test, we downloaded a subset of the dataset consisting of three particular classes of ``elementary shapes'': circle, square and triangle, and eliminated those sequences with length more than 20 time-steps.\footnote{The data provider noted that each object class might contain inappropriate content, for example straight lines and/or incomplete drawings.} This results in (CHECK HERE) 120,000 sequences for training. Then we use the code from \cite{ha2018sketch} for data-preprocessing\footnote{\url{https://github.com/tensorflow/magenta/tree/master/magenta/models/sketch_rnn}} and ignore the timestamps, which makes a sequence $\x_{1:T}$ be a list of 5-dimensional vectors: $\x_t = (\Delta x, \Delta y, p_1, p_2, p_3)$. Here $(\Delta x, \Delta y)$ is the offset of the pen from the previous drawing position, and $(p_1, p_2, p_3)$ is a one-hot vector indicating that the pen is either touching the paper now for $(1, 0, 0)$, or lifted from the paper for $(0, 1, 0)$. The third pen state $(0, 0, 1)$ denotes that the drawing has ended. 

\paragraph{Network architecture.}
The network architectures remains almost identical to the previous experiments, except that we set the hidden layer size to be 256, and the dimensionality of $\f$ and $\z_t$ to be 64. Also instead of Gaussian likelihood, we follow \cite{graves2013generating, ha2018sketch} to use a mixture density network \citep{bishop1994mixture} to define $p(\x_t | \z_t, \f)$, which is then a mixture of 10 Gaussian distributions. We find it useful to use warm-up \citep{sonderby2016ladder} at the beginning of the training, i.e.~we scale the $KL[q||p]$ terms in the variational lower-bound and increase the scale from 0 to 1 in the first 10,000 training iterations.

\paragraph{Qualitative analysis.}


